Scheduling Quantum Teleportation with Noisy Memories

Quantum teleportation channels can overcome the effects of photonic loss, a major challenge in the implementation of a quantum network over fiber. Teleportation channels are created by distributing an entangled state between two nodes which is a probabilistic process requiring classical communication. This causes critical delays that can cause information loss as quantum data suffers from decoherence when stored in memory. In this work, we quantify the effect of decoherence on fidelity at a node in a quantum network due to the storage of qubits in noisy memory platforms. We model the memory platform as a buffer that stores incoming qubits waiting for the creation of a teleportation channel. Memory platforms are parameterized with decoherence rate and buffer size, in addition to the order in which the incoming qubits are served. We show that fidelity at a node is a linear sum of terms, exponentially decaying with time, where the decay rate depends on the decoherence rate of the memory platform. This allows us to utilize Laplace Transforms to derive efficiently computable functions of average fidelity with respect to the load, buffer size, and decoherence rate of the memory platform. We prove that serving qubits in a Last In First Out order with pushout for buffer overflow management is optimal in terms of average fidelity. Lastly, we apply this framework to model a single repeater node to calculate the average fidelity of the teleportation channels created by this repeater assuming perfect gate operations.

==> optimality.tex <==
\section{Optimality of LIFO-PO}

We assume that jobs labelled $1,2,\ldots$ arrive to a system with a finite buffer of size $B$ at times $a_1 = 0 < a_2 < \cdots < a_i < \cdots $.  Assume requests can be served at times $0 < s_1 < \cdots < s_i < \cdots $. Here service corresponds to matching a job to a service time at which point, the job is instantly served and immediately departs the system.  Note that it is possible for the buffer to be full when a job arrives in which case the policy must decide whether or not to admit the job and if so, what job in the buffer to remove. Let $\pi$ denote the policy that assigns requests to service times and, decides when to remove requests from the buffer to avoid overflow.  If $\pi$ assigns job $i$ to service time $s_j$, we denote this decision as $\pi(i) = j$. If $\pi$ removes job $i$ from the buffer, we denote the decision by $\pi(i) = \Lambda$. As we are interested in maximizing the rate at which we serve jobs, it suffices to consider {\em work conserving policies}, and buffer management policies that makes removal decisions only at times that jobs arrive to find full buffers. A policy is said to be work conserving if it serves of jobs as early as possible.  Hence we restrict ourselves to the class of work conserving policies $\Pi$.   We introduce $\text{\LP}$, which always assigns the youngest job to the next service time and always throws out the oldest job from the buffer whenever the buffer is about to overflow. 

Let $d_j$ refer to the time that job $j$ is either served, $d_j = s_{\pi(j)}$ or removed, $\pi(j) = \Lambda$, and let $r_j$ denote the event, $r_j = 0$ if $\pi(j) \ne \Lambda$, $r_j = 1$ if $\pi(j) = \Lambda$,  $j=1,\ldots $.  {\LP} satisfies the following: 
\begin{itemize}
    \item There exists no pair of jobs, $j,k$, such that  $a_k < a_j < d_k < d_j$.
\end{itemize}  
 
Henceforth we refer to {\LP} as $\gamma$.
Consider $\pi \in \Pi$.  Of the first $n$ departures, $m\le n$ will be served and the remaining jobss will be thrown out.  Let $w^\pi = (w^\pi_1, \ldots ,w^\pi_n)$ denote the wait times of these jobs. Because jobs can be removed from the buffer without service, we will assign wait times of infinity to those jobs. 
Our proof that $\gamma$ is optimal is based on establishing a majorization result between $w^\pi$ and $w^\gamma$, $\pi \in \Pi$, $\pi \ne \gamma$. 
\begin{definition}
Let $x,y\in\R_+^n\times\{\infty\}^m$. $y$ majorizes $x$ written $x\prec y$ iff
\begin{align*} 
  \sum_{i=1}^k x_{(i)} \ge & \sum_{i=1}^k y_{(i)}, \quad k=1,\ldots , n-1\\
  \sum_{i=1}^n x_{(i)} = &\sum_{i=1}^n y_{(i)}
\end{align*}  
where $x_{(i)}$ (resp. $y_{(i)}$) correspond to the components of $x$ ($y$) in increasing order.\\
$y$ weakly supermajorizes $x$ written $x\wsm y$ iff
\[
  \sum_{i=1}^k x_{(i)} \ge \sum_{i=1}^ky_{(i)}, \quad k=1,\ldots , n.
\]
\end{definition}
Note that the standard definition corresponds to the case $m=0$. We introduce an operator $T_{ij}$, called the "$T$-transform", as follows.  Let $x\in \R_+^n$, then
\[ 
T_{ij} = \lambda I + (1-\lambda )Q_{ij}
\]
where $I$ is the identity operator, $Q_{ij}$ is an operator that permutes the $i$-th and $j$-th components of $X$ and $0\le \lambda \le 1$.  In other words,
\begin{align*}
T_{ij}x &= (x_1,\ldots ,x_{i-1},\lambda x_i +(1-\lambda)x_j,x_{i+1}, \ldots, \\
& x_{j-1},(1-\lambda)x_i + \lambda x_j,x_{j+1}, \ldots , X_n)
\end{align*}
It is easily shown that $T_{ij}x \prec x$ and $T_{ij}x \wsm x$ provided $x_i,x_j < \infty$.  Note that $x \prec Q_{ij}x$ and $x \wsm Q_{ij}x$ ($\lambda = 0$). Last, define the function $S_j(x)$ as
\[
 S_j(x) = (x_1,\ldots , s_{j-1},\alpha s_j,s_{j+1}, \ldots , s_n)
 \]
 with $0<\alpha < 1$.  Then $x \wsm S_j(x)$.
 
 A particularly useful property of $\wsm$ is the following, 
 \beq \label{eq:cxequiv}
 \sum_{i=1}^n \phi(x_{(i)}) \le \sum_{i=1}^n \phi(y_{(i)})
 \eeq
 for any continuous decreasing convex function $\phi$.
 
 Consider the first $n$ jobs $\cS = \{i_1, i_2, \ldots ,i_n\}$ that depart under $\pi$ at times $d^\pi_{i_1} < d^\pi_{i_2} < \cdots < d^\pi_{i_n}$.  
 %$d_1$ $e_1,\ldots ,e_u$ denote the different events up through the $n$-th departure.  Here $e_i = (t_i, j_i, v_i)$ where $t_i$ denote the time of the event, $j_i$ is the label of the request associated with the event, and $v_i$ denotes the type of event, $v_i \in\{a,d,r\}$ where $a$ denotes arrival, $d$ a departure,and $r$ removal from the buffer. We order the events such that {\em (i)} $t_1 \le t_2\le \cdots \le t_u$; and {\em (ii)} if $b_j = r$, then $b_{j-1} = a$ and the buffer is full at time $t_j$.
 
%Some additional notation.  Let $d_i$ and $r_i$ denote the departure and removal time of job $i$.  Note that job $i$ is either served or removed; hence we will overload this notation to allow $d_i = \Lambda$ to represent that $i$ was removed and $r_i = \Lambda$ to represent that $i$ was served.
 
 We now transform $\pi$ to $\gamma$ through a sequence of steps that each create a sequence of policies $\pi_0 = \pi, \pi_1, \pi_2, \ldots , \pi_h = \gamma$ such that $w^{\pi_l} \wsm w^{\pi_{l+1}}$, $l=0, \ldots h-1$.
 

 Assume that $\pi_l$ violates the above property of {\LP}. There are three cases depending on whether the two jobs are served, one is served and the other removed or both removed. In all three cases $a_k < a_j < d_k < d_j$ (we omit dependence on $\pi_l$).
 \begin{enumerate}
     \item {\bf Both are served.}  Job $k$ is served before a younger request $j$. We construct $\pi_{l+1}$ from $\pi_l$ by switching the order in which $j$ and $k$ are served. The wait times for jobs $j$ and $k$ under $\pi_l$ are $w^{\pi_l}_j = d_j - a_j$ and $w^{\pi_l}_k = d_k - a_k$ and under $\pi_{l+1}$ are $w^{\pi_{l+1}}_j = d_k - a_j$ and $w^{\pi_{l+1}}_k = d_j - a_k$. Here $w^{\pi_l}$ and $w^{\pi_{l+1}}$ satisfy
     \[
       w^{\pi_l} = T_{jk}w^{\pi_{l+1}} 
     \]
     with 
     \[
        \lambda = \frac{a_j - a_k} {(a_j-a_k)+(d_j - d_k)}.
     \]
     Hence $w^{\pi_l} \wsm w^{\pi_{l+1}}.$ See Figure \ref{fig:case1}.
     \item {\bf One job is served.}  job $k$ is served while a younger job is removed at a later time. We switch the order in which these two jobs are handled resulting in the servicing of $j$ at time $d_k$ and removal of $k$ at time $d_j$.   Then $w^{\pi_l} $ and $w^{\pi_{l+1}}$ satisfy
     \[
       w^{\pi_{l+1}} = S(Q_{jk}w^{\pi_l} )
     \]
     with $\alpha = (d_k - a_j)/(d_k - a_k).$
     Hence $w^{\pi_l} \wsm w^{\pi_{l+1}}.$
     \item {\bf Both are removed.} A younger job $j$ is removed from the buffer before an older job $k$ under $\pi_l$.  We switch the order of the removals under $\pi_{l+1}$.  This does not affect wait times and $w^{\pi_l} \wsm w^{\pi_{l+1}}.$
 \end{enumerate}
This procedure is repeated until the properties of $\LP$ are satisfied and, consequently $w^{\pi} \wsm w^{\gamma}$.

We fixed the arrival and service times. Remove the conditioning on them and let $W^{\pi}(n)$ denote the wait time of a randomly chosen request from the first $n$ requests that are served. From the above majorization result and the equivalence (\ref{eq:cxequiv}), we conclude that $\E [\phi (W^{\LP}(n)] \ge \E [\phi (W^{\pi}(n))]$ for every convex decreasing function $\phi$. Moreover if the limits $W^{\LP} = \lim_{n\rightarrow \infty} W^{\LP}(n)$ and $W^{\pi} = \lim_{n\rightarrow \infty} W^{\pi}(n)$ exist, then $\E [\phi (W^{\LP}] \ge \E [W^{\pi}]$.
\begin{figure}[ht]
\begin{subfigure}[b]{.5\textwidth}
\centerline{
		\begin{tikzpicture}[thick]
        \draw[thick] (1,0) -- (6.5,0) node[pos=0,left]{$\pi_l$};
        \draw[->,thick] (1.5,-0.5) -- (1.5,0) node[pos=0,right]{$a_k$};
        \draw[->,thick] (3,-0.5) -- (3,0) node[pos=0,right]{$a_j$};
        \draw[->,thick] (5,0) -- (5,0.5) node[pos=1,right]{$k$};
        \node at (5,-0.5) {$d_k$};
        \draw[->,thick] (6,0) -- (6,0.5)  node[pos=1,right]{$j$};
        \node at (6,-0.5) {$d_j$};
        \node (1) at (1.4,0.25){};
        \node (2) at (3.25,0.25) {$w_k^{\pi_l}$};
        \node (3) at (5.1,0.25){};
        \path[->]
        (2) edge (1) [thick] ;
        \path[->] (2) edge (3) [thick] ;
        \node (4) at (2.9,0.75){};
        \node (5) at (4.5,0.75) {$w_j^{\pi_l}$};
        \node (6) at (6.1,0.75){};
        \path[->]
        (5) edge (4) [thick] ;
        \path[->] (5) edge (6) [thick] ;
        \draw[thick] (1,-2) -- (6.5,-2) node[pos=0,left]{$\pi_{l+1}$}; 
        \draw[->,thick] (1.5,-2.5) -- (1.5,-2) node[pos=0,right]{$a_k$};
        \draw[->,thick] (3,-2.5) -- (3,-2) node[pos=0,right]{$a_j$};
        \draw[->,thick] (5,-2) -- (5,-1.5) node[pos=1,right]{$j$};
        \node at (5,-2.5) {$d_k$};
        \draw[->,thick] (6,-2) -- (6,-1.5) node[pos=1,right]{$k$};
        \node at (6,-2.5) {$d_j$};
        \node (7) at (1.4,-1.25){};
        \node (8) at (3.75,-1.25) {$w_k^{\pi_{l+1}}$};
        \node (9) at (5.1,-1.75){};
        \node (10) at (2.9,-1.75){};
        \node (11) at (4,-1.75) {$w_j^{\pi_{l+1}}$};
        \node (12) at (6.1,-1.25){};
        \path[->]
        (11) edge (10) [thick] ;
        \path[->] (11) edge (9) [thick] ;
        \path[->]
        (8) edge (7) [thick] ;
        \path[->] (8) edge (12) [thick] ;
		\end{tikzpicture}
}
        \caption{Case 1.}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
\centerline{
		\begin{tikzpicture}[thick]
        \draw[thick] (1,0) -- (6.5,0) node[pos=0,left]{$\pi_l$};
        \draw[->,thick] (1.5,-0.5) -- (1.5,0) node[pos=0,right]{$a_k$};
        \draw[->,thick] (3,-0.5) -- (3,0) node[pos=0,right]{$a_j$};
        \draw[->,thick] (5,0) -- (5,0.5) node[pos=1,right]{$k$};
        \node at (5,-0.5) {$d_k$};
%        \draw[->,thick] (6,0) -- (6,0.5)  node[pos=1,right]{$i$};
        \node at (6,0.5) {$j$};
        \node at (6,0) {\textcolor{red}{\bf{\sf X}}};
        \node at (6,-0.5) {$d_j$};
        \node (1) at (1.4,0.4){};
        \node (2) at (3.25,0.4) {$w_k^{\pi_l}$};
        \node (3) at (5.1,0.4){};
        \path[->]
        (2) edge (1) [thick] ;
        \path[->] (2) edge (3) [thick] ;
        \draw[thick] (1,-2) -- (6.5,-2) node[pos=0,left]{$\pi_{l+1}$}; 
        \draw[->,thick] (1.5,-2.5) -- (1.5,-2) node[pos=0,right]{$a_k$};
        \draw[->,thick] (3,-2.5) -- (3,-2) node[pos=0,right]{$a_j$};
        \draw[->,thick] (5,-2) -- (5,-1.5) node[pos=1,right]{$j$};
        \node at (5,-2.5) {$d_k$};
        \node at (6,0-1.5) {$k$};
        \node at (6,-2) {\textcolor{red}{\bf{\sf X}}};
        \node at (6,-2.5) {$r_j$};
        \node (9) at (5.1,-1.6){};
        \node (10) at (2.9,-1.6){};
        \node (11) at (4,-1.6) {$w_j^{\pi_{l+1}}$};
        \path[->]
        (11) edge (10) [thick] ;
        \path[->] (11) edge (9) [thick] ;
		\end{tikzpicture}
}
		\caption{Case 2.}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\centerline{
		\begin{tikzpicture}[thick]
        \draw[thick] (1,0) -- (6.5,0) node[pos=0,left]{$\pi_l$};
        \draw[->,thick] (1.5,-0.5) -- (1.5,0) node[pos=0,right]{$a_k$};
        \draw[->,thick] (3,-0.5) -- (3,0) node[pos=0,right]{$a_j$};
        \node at (5,0.5) {$j$};
        \node at (5,0) {\textcolor{red}{\bf{\sf X}}};
        \node at (5,-0.5) {$d_j$};
        \node at (6,0.5) {$k$};
        \node at (6,0) {\textcolor{red}{\bf{\sf X}}};
        \node at (6,-0.5) {$d_k$};
        \draw[thick] (1,-2) -- (6.5,-2) node[pos=0,left]{$\pi_{l+1}$}; 
        \draw[->,thick] (1.5,-2.5) -- (1.5,-2) node[pos=0,right]{$a_k$};
        \draw[->,thick] (3,-2.5) -- (3,-2) node[pos=0,right]{$a_j$};
        \node at (5,-1.5) {$k$};
        \node at (5,-2) {\textcolor{red}{\bf{\sf X}}};
        \node at (5,-2.5) {$d_j$};
        \node at (6,0-1.5) {$j$};
        \node at (6,-2) {\textcolor{red}{\bf{\sf X}}};
        \node at (6,-2.5) {$d_k$};
		\end{tikzpicture}
}
		\caption{Case 3.}
\end{subfigure}
\caption{Case 1: Effect of interchanging serving of two requests $i$ and $j$ when the properties of  {\LP}  are violated.} \label{fig:case1}
\end{figure}

\paragraph{Example: Application to a double buffer teleportation system}  Consider an end system with a stream of arriving teleportation requests whose qubits are placed in a memory of size $B_r$ and a stream of arriving EPR pairs whose qubits are placed in a memory of size $B_e$. Let $\Pi$ denote the set of double queue work conserving policies that only remove qubits when buffers are about to overflow.
Consider a policy $\pi \in \Pi$. When applied to the above system, the system behavior under $\pi$ can be visualized as a sequence of {\em service cycles} separated by idle periods (see Figure \ref{fig:service-cycles}). There are two types of service cycles as described next depending on whether request qubits  are stored waiting for EPR pairs or vice versa. A request (resp. EPR) cycle is a contiguous period of time when there is at least one request (resp. EPR) qubit stored in the request (resp. EPR) buffer. Note that there are no stored EPR qubits during a request cycle and vice versa. Its behavior is illustrated in \ref{fig:service-cycles}. Note that, the behavior illustrated in Fig. \ref{fig:service-cycles} is the same for all policies in $\Pi$. Only the identities of qubits being matched or removed from buffers are affected. 
Assume arrivals of request qubits and EPR qubits are characterized by Poisson processes with rates $\lambda_r$ and $\lambda_e$.  The Poisson assumption allows us to decompose the system into two subsystems, on focused on buffering of request qubits, the other focused on buffering of EPR qubits.  More specifically, when we focus on the first, we ignore all request qubits that arrive to find an EPR qubit available for teleportation And only consider those qubits that require buffering. As we will observe in Section ???, this modified system can be modeled as a continuous time Markov chain and request qubits will be characterized by a stationary wait time $W^\pi_r$.  Similarly, EPR qubits that require buffering are characterized by a stationary wait time $W^\pi_e$.  Assume that qubits decohere at different rates in the two memories, and the fidelity of a request qubit and an EPR qubit are $F_r(t)$ and $F_e(t)$ after storage for time $t$ respectively. Further assume $F_r(t)$ and $F_e(t)$ are decreasing convex functions in $t$. The results in this section allow us to conclude that  $\E [F_r (W^{\LP}(n)] \ge \E [F_r (W^{\pi}(n))]$ and $\E [F_e (W^{\LP}(n)] \ge \E [F_e (W^{\pi}(n))]$. The expected teleportation fidelity for the entire system, $\E[F^\pi]$ is $\E[F^\pi] = q\E[F^\pi] + (1-q) \E[F^\pi]$ where  $q$ is the probability that a request qubit arrives to a system where no EPR qubits are available.  Finally, we conclude $\E[F^{\LP}] \ge \E[F^\pi]$ for all $\pi \in \Pi$.
\begin{figure}[t]%{.5\textwidth}
\centerline{
		\begin{tikzpicture}[thick]
        \draw[->,thick] (1,0) -- (12,0) ;
        \draw[blue,thick] (1.5,0) -- (1.5,0.4) ;
        \draw[blue,thick] (1.5,0.4) -- (2.1,0.4) ;
        \draw[blue,thick] (2.1,0.4) -- (2.1,0.8) ;
        \draw[blue,thick] (2.1,0.8) -- (2.9,0.8) ;
        \draw[blue,thick] (2.9,0.8) -- (2.9,1.2) ;
        \draw[blue,thick] (2.9,1.2) -- (3.8,1.2) ;
        \draw[blue,thick] (3.8,1.2) -- (3.8,0.8) ;
        \draw[blue,thick] (3.8,0.8) -- (4.2,0.8) ;
        \draw[blue,thick] (4.2,0.8) -- (4.2,0.4) ;
        \draw[blue,thick] (4.2,0.4) -- (5.2,0.4) ;
        \draw[blue,thick] (5.2,0.4) -- (5.2,0) ;
        \node at (3.4,.25) {\color{blue}Request cycle};
        \draw[red,thick] (6.5,0) -- (6.5,0.4) ;
        \draw[red,thick] (6.5,0.4) -- (7.1,0.4) ;
        \draw[red,thick] (7.1,0.4) -- (7.1,0.8) ;
        \draw[red,thick] (7.1,0.8) -- (7.9,0.8) ;
        \draw[red,thick] (7.9,0.8) -- (7.9,1.2) ;
        \draw[red,thick] (7.9,1.2) -- (8.8,1.2) ;
        \draw[red,thick] (8.8,1.2) -- (8.8,0.8) ;
        \draw[red,thick] (8.8,0.8) -- (9.2,0.8) ;
        \draw[red,thick] (9.2,0.8) -- (9.2,0.4) ;
        \draw[red,thick] (9.2,0.4) -- (10,0.4) ;
        \draw[red,thick] (10,0.4) -- (10,0.8) ;
        \draw[red,thick] (10,0.8) -- (10.4,0.8) ;
        \draw[red,thick] (10.4,0.8) -- (10.4,0.4) ;
        \draw[red,thick] (10.4,0.4) -- (11.2,0.4) ;
        \draw[red,thick] (11.2,0.4) -- (11.2,0) ;
        \node at (8.4,.25) {\color{red}EPR cycle};
        \node at (11,-0.3) {$t$};
		\end{tikzpicture}
}
        \caption{Typical teleportation behavior.} \label{fig:service-cycles}
\end{figure}
